Joint Optimization of Tree-based Index and Deep Model for Recommender Systems

Large-scale industrial recommender systems are usually confronted with computational problems due to the enormous corpus size. To retrieve and recommend the most relevant items to users under response time limits, resorting to an efficient index structure is an effective and practical solution. The previous work Tree-based Deep Model (TDM) \cite{zhu2018learning} greatly improves recommendation accuracy using tree index. By indexing items in a tree hierarchy and training a user-node preference prediction model satisfying a max-heap like property in the tree, TDM provides logarithmic computational complexity w.r.t. the corpus size, enabling the use of arbitrary advanced models in candidate retrieval and recommendation. In tree-based recommendation methods, the quality of both the tree index and the user-node preference prediction model determines the recommendation accuracy for the most part. We argue that the learning of tree index and preference model has interdependence. Our purpose, in this paper, is to develop a method to jointly learn the index structure and user preference prediction model. In our proposed joint optimization framework, the learning of index and user preference prediction model are carried out under a unified performance measure. Besides, we come up with a novel hierarchical user preference representation utilizing the tree index hierarchy. Experimental evaluations with two large-scale real-world datasets show that the proposed method improves recommendation accuracy significantly. Online A/B test results at a display advertising platform also demonstrate the effectiveness of the proposed method in production environments.

==> section2.tex <==
\section{Related Work} \label{section:RelatedWork}
In real-world applications, the recommendation process usually has two stages: candidate generation and ranking \cite{davidson2010youtube, zhu2018learning, OCPC}.
Model-based large-scale recommendation methods are usually confronted with computational restrictions in the candidate generation stage.
To overcome the calculation barrier, there are mainly three kinds of approaches: 
1) Pre-calculate item or user similarities and use inverted index to accelerate the retrieval \cite{linden2003amazon};
2) Convert user preference to distance of embedding vectors, and use approximate kNN search in retrieval \cite{Covington2016Deep};
3) Use tree or ensemble of trees to perform efficient retrieval \cite{zhu2018learning}.

% introduce vector based method

Industrial recommender systems typically adopt vector kNN search to achieve fast retrieval, e.g., 
YouTube video recommendation \cite{Covington2016Deep, beutel2018latent}, Yahoo news recommendation \cite{okura2017embedding}
and extensions that use recurrent neural network to model user behavior sequence \cite{hidasi2015session, tan2016improved, wu2017recurrent}.
Such approaches use either traditional deep neural network (DNN) or recurrent neural network (RNN) to learn user and item's embedding representations based on various user behavioral and contextual data.
However, due to the dependence of approximate kNN search index structures in retrieval, 
user preference models that use attention network or cross features \cite{zhou2018deep1, zhou2018deep, cheng2016wide} are challenging to be applied.
%in vector kNN search based methods, which limits the accuracy of user preference prediction.

% introduce other tree-based method

Tree-based methods are also studied and adopted in real-world applications.
Label Partitioning for Sublinear Ranking (LPSR) \cite{weston2013label} uses k-means clustering with data points' features
to learn the tree hierarchy and then assign labels to leaf nodes.
In the prediction stage, the test sample is passed down along the tree to a leaf node according to its distance to each node's cluster center, 
and the 1-vs-All base classifier is used to rank all labels belonged to the retrieved leaf node.
Partitioned Label Trees (Parabel) \cite{prabhu2018parabel} also use recursive clustering to build tree hierarchy, but the tree is built to partition the labels according to label similarities.
Multi-label Random Forest (MLRF) \cite{agrawal2013multi} and FastXML \cite{prabhu2014fastxml} learn an ensemble of sample partitioning trees (a forest), 
and a ranked list of the most frequent labels in all the leaf nodes retrieved from the forest is returned in prediction.
MLRF optimizes the Gini index when splitting nodes, and FastXML optimizes a combined loss function including a binary classification loss and a label ranking loss.
In all the above methods, the tree structure keeps unchanged in training and prediction once built, 
which is hard to completely adapt the retrieval model dynamically.
%TDM \cite{zhu2018learning} gives a solution that uses items' category information to construct the initial tree to train the user-node preference model.
%And after training the model, the learnt item embedding vectors are used to build a new tree by recursive k-means clustering \cite{macqueen1967some, mnih2009scalable, pmlr-v80-han18a, chen2018large, prabhu2018parabel}.

%Tree-based recommendation methods are also studied as equivalent to extreme classification problem.
%Label Partition for Sublinear Ranking (LPSR) \cite{weston2013label} use hierarchical clustering to split samples into partitions according to their features.
%%However, such feature vector clustering based sample partitioning is not a good solution in recommendation, because the user feature vector may change with the training of user preference model.
%Multi-label Random Forest (MLRF) \cite{agrawal2013multi} and FastXML \cite{prabhu2014fastxml} both use ensemble of trees, but they use different node splitting methods in the tree learning stage.
%MLRF optimizes the Gini index when splitting nodes, and FastXML optimizes a combined loss function including a binary classification loss and a label ranking loss.
%%Both MLRF and FastXML focus more on performing classification in each non-leaf node but do not directly model the user-node preference.
%Partitioned Label Trees (Parabel) \cite{prabhu2018parabel} uses recursive clustering to partition the label space according to label similarities.
%In all the above methods, the tree structure keeps unchanged in training and prediction once has been built, 
%which is hard to cooperate the dynamic model training process.

% introduce TDM

Our previous work TDM \cite{zhu2018learning} introduces a tree-based model for large-scale recommendation  
differentiated from existing tree-based methods with a max-heap like user-node preference formulation.
In TDM, tree is used as a hierarchical index \cite{kraska2018case}, and an attention model \cite{zhou2018deep1} is trained to predict user-node preference.
Different from most tree-based methods where non-leaf nodes are used to route decision-making to leaves, 
TDM explicitly formulates user-node preference for all the nodes to facilitate hierarchical beam search in the tree index.
Despite achieving remarkable progress, 
the joint optimization problem of index and model is not well solved yet as that the proposed alternatively learning method of model and tree has different objectives.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figure/tdm_plus_plus.eps}
\caption{Tree-based deep recommendation model. (a) User preference prediction model. We firstly hierarchically abstract the user behaviors with nodes in corresponding layers. Then the abstract user behaviors and the target node together with the other feature such as the user profile are used as the input of the model. (b) Tree hierarchy. Each item is firstly assigned to a different leaf node with a projection function $\pi(\cdot)$. Red nodes (items) in the leaf level are selected as the candidate set.}\label{fig:tdm_plus}
\end{figure}
%In most of the other tree-based works, node-specific classifiers are trained, 
%to decide in each node that which children of the node should the test samples be passed to.
%While in TDM, user-node preference for each non-leaf node is directly formulated and estimated to perform hierarchical beam search in the tree index.
%In training stage, TDM uses items' category information to construct the initial tree to train the user-node preference model.
%And after training the model, the learnt item embedding vectors are used to build a new tree by recursive k-means clustering \cite{macqueen1967some, mnih2009scalable, pmlr-v80-han18a, chen2018large, prabhu2018parabel}.
%Despite achieving remarkable progress, the joint optimization problem of index and model is not well solved yet as that the alternatively learning process of model and tree has different objectives.

%Our previous work TDM \cite{zhu2018learning} introduces a tree-based framework for large-scale recommendation problem, 
%where tree is used as a hierarchical index \cite{kraska2018case} to make recommendation with any advanced user preference prediction model computational tractable.
%TDM differs from other tree-based works mainly on its max-heap like hierarchical user-node preference formulation.
%In TDM's formulation, each non-leaf node's user-node preference is supposed as the larger one of its children's preferences like a max-heap,
%and a global user-node preference model is trained to fit such a preference distribution.
%Compared to other tree-based works that the tree nodes are regarded as routes to pass samples down to the leaf, TDM directly models user-node preference for each node in the tree.
%In prediction stage, the model given preference score is used to perform layer-wise beam-search to retrieve user's most interested leaf nodes, i.e., items.
%Despite achieving remarkable progress, the joint optimization problem of index and model is not well solved yet.


==> section4.tex <==
\section{Task-oriented Learning Approach} \label{section:TaskOrientedLearning}
Introduce the ECPM maximization demands in online display advertising (cost-per-click ads) and show how to solve the problem in candidate generation stage using TDM framework.

